AdapterBias: Parameter-efficient Token-dependent Representation Shift for Adapters in NLP Tasks

Transformer-based pre-trained models with millions of parameters require large storage. Recent approaches tackle this shortcoming by training adapters, but these approaches still require a relatively large number of parameters. In this study, AdapterBias, a surprisingly simple yet effective adapter architecture, is proposed. AdapterBias adds a token-dependent shift to the hidden output of transformer layers to adapt to downstream tasks with only a vector and a linear layer. Extensive experiments are conducted to demonstrate the effectiveness of AdapterBias. The experiments show that our proposed method can dramatically reduce the trainable parameters compared to the previous works with a minimal decrease in task performances compared with fine-tuned pre-trained models. We further find that AdapterBias automatically learns to assign more significant representation shifts to the tokens related to the task in consideration.

==> Figures/sparse.tex <==
\begin{figure}
    \centering
      \includegraphics[width=0.47\textwidth]{Figures/sparse.png}
      %\caption{model architecture of vector linear}
      \caption{We drop partial of parameter in the inference time. In this figure, we use BERT-base model and report the GLUE average score in validation data. The x-axis represents the ratio of dropping parameter to total parameter, which is available to drop. We define three dropping approaches here: Drop $v+L$, Drop $v$ and Drop $L$. We drop different components in these approaches.}
      \label{fig:drop}
\end{figure}

==> Tables/explain.tex <==

\begin{table*}[h]

\centering
\resizebox{\textwidth}{8mm}{
\begin{tabular}{c|ccccccccccc}
\hline
\small\textbf{Task}&
\small\text{'he'}&\small\text{'is'}&\small\text{'a'}&\small\text{'good'}&\small\text{'person'}&\small\text{'and'}&\small\text{'is'}&\small\text{'kind'}&\small\text{'to'}&\small\text{'everyone'}&\small\text{'.'}\\
\hline 
\small{CoLA}
&\small\text\textcolor{mycolor2}{7.25}%3
&\small\text\textcolor{mycolor5}{6.69}%4
&\small\text\textcolor{mycolor2}{7.68}%2
&\small\text\textcolor{mycolor4}{4.89}%11
&\small\text\textcolor{mycolor4}{5.14}%10
&\small\text\textcolor{mycolor5}{6.59}%6
&\small\text\textcolor{mycolor5}{6.65}%5
&\small\text\textcolor{mycolor3}{6.43}%8
&\small\text\textcolor{mycolor3}{6.27}%9
&\small\text\textcolor{mycolor3}{6.49}%7
&\small\textcolor{mycolor1}{11.92} %1
\\
\hline 
\small{SST-2}
&\small\text\textcolor{mycolor3}{13.79}%8
&\small\text\textcolor{mycolor3}{14.74}%7
&\small\text\textcolor{mycolor2}{16.41}%3
&\small\text\textcolor{mycolor2}{18.7}%2
&\small\text\textcolor{mycolor3}{13.56}%9
&\small\text\textcolor{mycolor5}{16.01}%4
&\small\text\textcolor{mycolor5}{15.85}%5
&\small\text\textcolor{mycolor5}{15.48}%6
&\small\text\textcolor{mycolor4}{11.18}%11
&\small\text\textcolor{mycolor4}{11.88}%10
&\small\text\textcolor{mycolor1}{20.72}%1
\\
\hline
\end{tabular}}
\caption{Results on the weigh change of same sentence in different tasks.}
\label{tab:dif}
\end{table*}


\begin{table*}[h]
\vspace*{-5pt}
\centering
\resizebox{\textwidth}{10mm}{
\begin{tabular}{c|ccccccccccc|c}
\hline
\small\textbf{Sentence 1}&
\small\text{'he'}&\small\text{'is'}&\small\text{'a'}&\small\text{'good'}&\small\text{'person'}&\small\text{'and'}&\small\text{'is'}&\small\text{'kind'}&\small\text{'to'}&\small\text{'everyone'}&\small\text{'.'}&\small\text{Prediction}\\
\hline 
%\multirow{3}{*}{CoLA}
\small{value}
&\small\text\textcolor{mycolor2}{7.25}%3
&\small\text\textcolor{mycolor3}{6.69}%4
&\small\text\textcolor{mycolor2}{7.68}%2
&\small\text\textcolor{mycolor5}{4.89}%11
&\small\text\textcolor{mycolor5}{5.14}%10
&\small\text\textcolor{mycolor3}{6.59}%6
&\small\text\textcolor{mycolor3}{6.65}%5
&\small\text\textcolor{mycolor4}{6.43}%8
&\small\text\textcolor{mycolor4}{6.27}%9
&\small\text\textcolor{mycolor4}{6.49}%7
&\small\textcolor{mycolor1}{11.92} %1
&\small{True}\\
\hline
 
\small\textbf{Sentence 2}&
\small\text{'he'}&\small\text{'will'}&\small\text{'a'}&\small\text{'good'}&\small\text{'person'}&\small\text{'and'}&\small\text{'is'}&\small\text{'kindly'}&\small\text{'to'}&\small\text{'everyone'}&\small\text{'.'}&\small\text{Prediction}\\
\hline
\small{value}
&\small\text\textcolor{mycolor1}{7.7}%3
&\small\text\textcolor{mycolor2}{6.79}%6
&\small\text\textcolor{mycolor1}{8}%2
&\small\text\textcolor{mycolor3}{5.56}%10
&\small\text\textcolor{mycolor3}{5.84}%11
&\small\text\textcolor{mycolor4}{6.15}%9
&\small\text\textcolor{mycolor4}{6.64}%7
&\small\text\textcolor{mycolor2}{7.6}%4
&\small\text\textcolor{mycolor2}{7.2}%5
&\small\text\textcolor{mycolor4}{6.29}%8
&\small\text\textcolor{mycolor1}{11.66}%1
&\small{False}\\
\hline
\end{tabular}}
\caption{Results on the weight change of different sentences in CoLA task.}
\label{tab:same}
\end{table*}


==> Tables/only_vector.tex <==
\begin{table*}[h]
\resizebox{\textwidth}{8mm}{
\begin{tabular}{c|l|c|cccccccccc}
\hline
\multicolumn{2}{c|}{\textbf{Method}} & \textbf{Params/task} & \textbf{COLA} & \textbf{SST-2} & \textbf{MRPC} & \textbf{QNLI} & \textbf{RTE} & \textbf{STS-B} & \textbf{MNLI-m} & \textbf{MNLI-mm} & \textbf{QQP} & \textbf{Avg} \\ \hline
\multicolumn{2}{c|}{Only \textit{vector}}     & \textbf{0.008}\%               & 45.6          & 91.5           & 87.4          & 88.3          & 65.6         & 81.0           & 77.9            & 78.4             & 65.7         & 75.7         \\
\multicolumn{2}{c|}{\textbf{AdapterBias}}             & 0.075\%              & \textbf{51.6}          & \textbf{93.1}           & \textbf{87.5}          & \textbf{89.4}          & \textbf{66.1}         & \textbf{84.6}           & \textbf{80.9}            & \textbf{80.5}             & \textbf{67.9}         & 
\textbf{78.0}  \\
\hline
\end{tabular}}
\caption{Analysis of AdapterBias without the linear layer ($L$), which produces $\alpha$. We report the total number of trainable parameters per task and results are on GLUE validation sets. The backbone model is BERT-base. Only $vector$ means that we remove $L$ and thus the embedding shift is equivalent among each token.}
\label{tb:onlyvector}
\end{table*}

==> tables.tex <==




\begin{table*}[h]
\vspace*{-15pt}
\centering
\resizebox{\textwidth}{8mm}{
\begin{tabular}{c|ccccccccccc}
\hline
\small\textbf{Task}&
\small\text{'he'}&\small\text{'is'}&\small\text{'a'}&\small\text{'good'}&\small\text{'person'}&\small\text{'and'}&\small\text{'is'}&\small\text{'kind'}&\small\text{'to'}&\small\text{'everyone'}&\small\text{'.'}\\
\hline 
\small{CoLA}
&\small\text\textcolor{mycolor2}{7.25}%3
&\small\text\textcolor{mycolor5}{6.69}%4
&\small\text\textcolor{mycolor2}{7.68}%2
&\small\text\textcolor{mycolor4}{4.89}%11
&\small\text\textcolor{mycolor4}{5.14}%10
&\small\text\textcolor{mycolor5}{6.59}%6
&\small\text\textcolor{mycolor5}{6.65}%5
&\small\text\textcolor{mycolor3}{6.43}%8
&\small\text\textcolor{mycolor3}{6.27}%9
&\small\text\textcolor{mycolor3}{6.49}%7
&\small\textcolor{mycolor1}{11.92} %1
\\
\hline 
\small{SST-2}
&\small\text\textcolor{mycolor3}{13.79}%8
&\small\text\textcolor{mycolor3}{14.74}%7
&\small\text\textcolor{mycolor2}{16.41}%3
&\small\text\textcolor{mycolor2}{18.7}%2
&\small\text\textcolor{mycolor3}{13.56}%9
&\small\text\textcolor{mycolor5}{16.01}%4
&\small\text\textcolor{mycolor5}{15.85}%5
&\small\text\textcolor{mycolor5}{15.48}%6
&\small\text\textcolor{mycolor4}{11.18}%11
&\small\text\textcolor{mycolor4}{11.88}%10
&\small\text\textcolor{mycolor1}{20.72}%1
\\
\hline
\end{tabular}}
\caption{Results on the weigh change of same sentence in different tasks.}
\label{tab:accents}
\end{table*}


\begin{table*}[h]
\vspace*{-5pt}
\centering
\resizebox{\textwidth}{10mm}{
\begin{tabular}{c|ccccccccccc|c}
\hline
\small\textbf{Sentence 1}&
\small\text{'he'}&\small\text{'is'}&\small\text{'a'}&\small\text{'good'}&\small\text{'person'}&\small\text{'and'}&\small\text{'is'}&\small\text{'kind'}&\small\text{'to'}&\small\text{'everyone'}&\small\text{'.'}&\small\text{Prediction}\\
\hline 
%\multirow{3}{*}{CoLA}
\small{value}
&\small\text\textcolor{mycolor2}{7.25}%3
&\small\text\textcolor{mycolor3}{6.69}%4
&\small\text\textcolor{mycolor2}{7.68}%2
&\small\text\textcolor{mycolor5}{4.89}%11
&\small\text\textcolor{mycolor5}{5.14}%10
&\small\text\textcolor{mycolor3}{6.59}%6
&\small\text\textcolor{mycolor3}{6.65}%5
&\small\text\textcolor{mycolor4}{6.43}%8
&\small\text\textcolor{mycolor4}{6.27}%9
&\small\text\textcolor{mycolor4}{6.49}%7
&\small\textcolor{mycolor1}{11.92} %1
&\small{True}\\
\hline
 
\small\textbf{Sentence 2}&
\small\text{'he'}&\small\text{'will'}&\small\text{'a'}&\small\text{'good'}&\small\text{'person'}&\small\text{'and'}&\small\text{'is'}&\small\text{'kindly'}&\small\text{'to'}&\small\text{'everyone'}&\small\text{'.'}&\small\text{Prediction}\\
\hline
\small{value}
&\small\text\textcolor{mycolor1}{7.7}%3
&\small\text\textcolor{mycolor2}{6.79}%6
&\small\text\textcolor{mycolor1}{8}%2
&\small\text\textcolor{mycolor3}{5.56}%10
&\small\text\textcolor{mycolor3}{5.84}%11
&\small\text\textcolor{mycolor4}{6.15}%9
&\small\text\textcolor{mycolor4}{6.64}%7
&\small\text\textcolor{mycolor2}{7.6}%4
&\small\text\textcolor{mycolor2}{7.2}%5
&\small\text\textcolor{mycolor4}{6.29}%8
&\small\text\textcolor{mycolor1}{11.66}%1
&\small{False}\\
\hline
\end{tabular}}
\caption{Results on the weight change of different sentences in CoLA task.}
\label{tab:accents}
\end{table*}

